FastVID: Dynamic Density Pruning for Fast Video Large Language Models

Video Large Language Models have demonstrated strong video understanding capabilities, yet their practical deployment is hindered by substantial inference costs caused by redundant video tokens. Existing pruning techniques fail to effectively exploit the spatiotemporal redundancy present in video data. To bridge this gap, we perform a systematic analysis of video redundancy from two perspectives: temporal context and visual context. Leveraging these insights, we propose Dynamic Density Pruning for Fast Video LLMs termed FastVID. Specifically, FastVID dynamically partitions videos into temporally ordered segments to preserve temporal structure and applies a density-based token pruning strategy to maintain essential spatial and temporal information. Our method significantly reduces computational overhead while maintaining temporal and visual integrity. Extensive evaluations show that FastVID achieves state-of-the-art performance across various short- and long-video benchmarks on leading Video LLMs, including LLaVA-OneVision, LLaVA-Video, Qwen2-VL, and Qwen2.5-VL. Notably, on LLaVA-OneVision-7B, FastVID effectively prunes $\textbf{90.3%}$ of video tokens, reduces FLOPs to $\textbf{8.3%}$, and accelerates the LLM prefill stage by $\textbf{7.1}\times$, while maintaining $\textbf{98.0%}$ of the original accuracy. The code is available at https://github.com/LunarShen/FastVID.

==> Fig/param_dyseg_stprune.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.49\textwidth}
        \begin{subfigure}[t]{.495\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Fig/Src/param_c.pdf}
            \caption{}
            \label{fig:param_c}
          \end{subfigure}
          \hfill
          \begin{subfigure}[t]{.495\linewidth}
            \centering
            \includegraphics[width=\linewidth]{Fig/Src/param_tau.pdf}
            \caption{}
            \label{fig:param_tau}
          \end{subfigure}
          \caption{Ablation study on $c$ and $\tau$ in DySeg. $c$ denotes the minimum number of segments in a video, whereas $\tau$ denotes the transition similarity threshold. Both parameters jointly control the segmentation granularity.}
          \label{fig:param_dyseg}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \begin{subfigure}[t]{.495\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Fig/Src/param_p.pdf}
    \caption{}
    \label{fig:param_p}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.495\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Fig/Src/param_beta.pdf}
    \caption{}
    \label{fig:param_beta}
  \end{subfigure}
  \caption{Ablation study on $p$ and $\beta$ in DTM. $p$ denotes the interval for anchor frame selection, whereas $\beta$ controls the merging weight for anchor tokens and their associated tokens in Eq. (\ref{eq:merge}).}
  \label{fig:param_stprune}
    \end{minipage}
\end{figure}

==> Tab/STPrune.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{c|ccccc}
\toprule
\multirow{2}{*}{\makecell{$d$\\in STPrune}} & \multirow{2}{*}{MVBench} & \multirow{2}{*}{\makecell{LongVideo-\\Bench}} & \multirow{2}{*}{MLVU} & \multirow{2}{*}{VideoMME} & \multirow{2}{*}{Avg.} \\
                         &                          &                                  &                       &                           &                       \\ \midrule
0.0/ATS                  & 55.3                     & 55.3                             & 62.4                  & 55.0                      & 96.2                  \\
0.2                      & 55.0                     & 53.6                             & 62.1                  & 56.1                      & 95.7                  \\
0.4                      & 55.9                     & \textbf{56.3}                             & \textbf{62.7}                  & \textbf{57.3}                      & \textbf{98.0}                  \\
0.6                      & 55.6                     & 54.5                             & 62.0                  & 56.2                      & 96.3                  \\
0.8                      & \textbf{56.0}                     & 54.9                             & 62.6                  & 55.6                      & 96.7                  \\
1.0/DTM                  & 54.1                     & 50.1                             & 61.5                  & 55.9                      & 93.5                  \\ \bottomrule
\end{tabular}
}
\caption{Ablation Study on $d$ in STPrune. STPrune consists of DTM and ATS. A fraction $d$ of the pruned tokens is from DTM, while the remaining $1-d$ is from ATS. When $d=0.0$, all pruned tokens are from ATS, while at $d = 1.0$, they are from DTM.}
\label{tab:stprune}
\end{table}

==> Tab/diffDTM.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}
{
\begin{tabular}{cccccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\makecell{Token\\Merging}}} & \multirow{2}{*}{MVBench} & \multirow{2}{*}{\makecell{LongVideo-\\Bench}} & \multirow{2}{*}{MLVU} & \multirow{2}{*}{VideoMME} & \multirow{2}{*}{Avg.} \\
\multicolumn{1}{c|}{}                     &                          &                                  &                       &                           &                       \\ \hline
\multicolumn{6}{c}{LLaVA-OneVision}                                                                                                                                                 \\ \hline
\multicolumn{1}{c|}{Uniform}              &	55.0	&	54.7	&	62.0	&	56.4	&	96.2                   \\
\multicolumn{1}{c|}{Cluster-based}        &	55.6	&	55.2	&	62.4	&	57.3	&	97.2                      \\
\multicolumn{1}{c|}{Our DTM}        & \textbf{55.9}                     & \textbf{56.3}                             & \textbf{62.7}                  & \textbf{57.3}                      & \textbf{98.0}                  \\ \hline
\multicolumn{6}{c}{LLaVA-Video}                                                                                                                                                     \\ \hline
\multicolumn{1}{c|}{Uniform}              &	55.4	&	54.6	&	62.9	&	59.8	&	91.5                       \\
\multicolumn{1}{c|}{Cluster-based}       &	55.3	&	55.1	&	62.9	&	60.1	&	91.8                       \\
\multicolumn{1}{c|}{Our DTM}        &	\textbf{58.5}	&	\textbf{56.5}	&	\textbf{64.9}	&	\textbf{60.7}	&	\textbf{94.7}
                   \\ \bottomrule
\end{tabular}
}
\caption{Ablation study on different token merging strategies. Uniform, adopted in VisionZip (see Figure~\ref{fig:intro_video_context}c), merges tokens through uniform sampling. Cluster-based methods (see Figure~\ref{fig:method_merge}a) conduct clustering algorithms. Our proposed DTM employs a density-based method (see Figure~\ref{fig:method_merge}b).}
\label{tab:diffdtm}
\end{table}

==> Tab/length.tex <==
\begin{table}[t]
\centering
\caption{Improved length extrapolation via FastVID. We report the overall performance of LLaVA-OneVision.}
\resizebox{0.50\linewidth}{!}
{
\begin{tabular}{c|cc|cc}
\toprule
Method  & \# Frame & \# Token & \multicolumn{2}{c}{VideoMME} \\ \midrule
\rowcolor{mygrayL} Vanilla & 32       & 6272     & 58.6         & 100\%           \\ \hline
FastVID (r=25\%) & 128      & 6272     & 60.4         & 103.1\%         \\
FastVID (r=10\%) & 320      & 6080     & 61.4         & 104.8\%         \\ \bottomrule
\end{tabular}
}
\label{tab:length}
\end{table}

==> Tab/more_sota_act.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\caption{Additional quantitative results on ANet-QA. We report the overall performance of LLaVA-OneVision.}
\resizebox{0.40\linewidth}{!}
{
\begin{tabular}{c|c|cc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{TFLOPs} & \multicolumn{2}{c}{ANet-QA} \\
                        &                         & Accuracy         & Score        \\ \midrule
\rowcolor{mygrayL} Vanilla                 & 48.82                   & 54.4             & 3.57         \\ \hline
PyramidDrop             & 14.70                   & 41.2             & 3.07         \\
\textbf{FastVID}                 & 4.04                    & \textbf{53.1}             & \textbf{3.52}         \\ \bottomrule
\end{tabular}
}
\label{tab:more_sota_act}
\end{table}

==> Tab/more_sota_ov.tex <==
\begin{table}[t]
\centering
\caption{Additional quantitative results on VideoMME. We report the overall performance of LLaVA-OneVision.}
\resizebox{0.60\linewidth}{!}
{
\begin{tabular}{c|cc|c}
\toprule
Method      & \makecell{Retention\\Ratio $R$} & TFLOPs & VideoMME \\ \midrule
\rowcolor{mygrayL} Vanilla     & 100\%             & 48.82  & 58.6     \\ \hline
PyramidDrop~\cite{xing2024pyramiddrop}$_{\text{CVPR'25}}$ & 100\%/4.1\%/2.0\%/1.0\% & 14.70  & 51.8     \\
SparseVLM$~\cite{zhang2024sparsevlm}_{\text{ICML'25}}$ & 100\%/10.4\%/5.3\%/2.9\% & 7.06	& 53.3 \\
LLaVA-PruMerge~\cite{shang2024llava}$_{\text{ICCV'25}}$ & 9.7\% & 4.04	& 49.9 \\
\textbf{FastVID}     & 9,7\%             & 4.04   & \textbf{57.3}     \\ \bottomrule
\end{tabular}
}
\label{tab:more_sota_ov}
\end{table}

==> Tab/sigliphead.tex <==
\begin{table}[t]
\centering
\caption{Ablation study on the SigLIP head. We report the overall performance of LLaVA-OneVision.}
\resizebox{0.35\linewidth}{!}
{
\begin{tabular}{c|c}
\toprule
Method  & VideoMME  \\ \midrule
FastVID & \textbf{57.3}  \\
w/o the SigLIP head & 56.3 \\ \bottomrule
\end{tabular}
}
\label{tab:sigliphead}
\end{table}
